DeepPicar: A Low-cost Deep Neural Network-based Autonomous Car

We present DeepPicar, a low-cost deep neural network based autonomous car platform. DeepPicar is a small scale replication of a real self-driving car called DAVE-2 by NVIDIA. DAVE-2 uses a deep convolutional neural network (CNN), which takes images from a front-facing camera as input and produces car steering angles as output. DeepPicar uses the same network architecture---9 layers, 27 million connections and 250K parameters---and can drive itself in real-time using a web camera and a Raspberry Pi 3 quad-core platform. Using DeepPicar, we analyze the Pi 3's computing capabilities to support end-to-end deep learning based real-time control of autonomous vehicles. We also systematically compare other contemporary embedded computing platforms using the DeepPicar's CNN-based real-time control workload. We find that all tested platforms, including the Pi 3, are capable of supporting the CNN-based real-time control, from 20 Hz up to 100 Hz, depending on hardware platform. However, we find that shared resource contention remains an important issue that must be considered in applying CNN models on shared memory based embedded computing platforms; we observe up to 11.6X execution time increase in the CNN based control loop due to shared resource contention. To protect the CNN workload, we also evaluate state-of-the-art cache partitioning and memory bandwidth throttling techniques on the Pi 3. We find that cache partitioning is ineffective, while memory bandwidth throttling is an effective solution.

==> discussion.tex <==
\section{Discussion}\label{sec:discussion}

In this section, we discuss issues that affect prediction accuracy and
real-time performance of the DeepPicar system.

\subsection{DNN Training and Testing}
We have trained and tested the deep neural network with several
different track conditions, different combinations of input
data, and different hyper parameters. In the following paragraphs, we 
describe details on two of the training methods that performed 
reasonably well.

\begin{figure}[h]
  \centering
  \includegraphics[width=1.0\textwidth, height=5cm]{figs/TrainingLoss}
  \caption{Change in loss value throughout training.}
  \label{fig:modelloss}
\end{figure}

In the first method, we trained the neural network model across a set 
of 30 completed runs on the track seen in Figure~\ref{fig:track} by a
human pilot. Half of the runs saw the car driving one way along the
track, while the remaining half were of the car driving in the
opposite direction on the track.
In total, we collected 2,481 frames for training and 2,534 
frames for validation.
The weights of the network are initialized using a Xavier
initializer~\cite{Glorot2010}, which is known to provide better
initial values than the random weight assignment method.
In each training step, we use a batch
size of 100 frames, which are randomly selected among all the
collected training images, to optimize the network.
We repeat this across 2,000 training steps. When a model was trained
with the  aformentioned data, the training loss was 0.0151 and the
validation  loss was 0.0251.
The change of the loss value over the course of model training can be
seen in Figure~\ref{fig:modelloss}.

In the second method, we use the same data and parameters as  above 
except that now images are labeled as 'curved' and 'straight' and we pick an
equal number of images from each category at each training step to
update the model. In other words, we try to remove bias in selecting
images. We find that the car performed better in practice by applying
this approach as the car displayed a greater ability to stay in the
center of the track (on the white tape).
However, we find that there is a huge discrepency between the training
loss and the validation loss as the former was 0.0126, while the latter
was 0.0725 --- almost a 6X difference---indicating that the model 
suffers from an overfitting problem.

We continue to investigate ways to achieve better prediction accuracy
in training the network, as well as improving the performance of the RC
car platform, especially related to precise steering angle control.

\subsection{System-level Factors Affecting Real-Time Performance}
In using the Raspberry Pi 3 platform, there are a
few system-level factors, namely power supply and temperature, that
need to be considered to achieve consistent and high real-time
performance. 

In all our experiments on the Raspberry Pi 3, the CPU  operated at a
preferred clock speed of 1.2 GHz. However, without care, it is
possible for the CPU to operate at a lower frequency. 

An important factor is CPU thermal throttling, which can affect CPU
clock speed if the CPU temperature is too high (Pi 3's firmware is
configured to throttle at 85C).
DNN model operations are computationally intensive, thus it is
possible for the temperature of the CPU to rise quickly. This can be
especially problematic in situations where multiple DNN models are
running simultaneously on the Pi 3.
If the temperature reaches the threshold, the Pi 3's thermal
throttling kicks in and decreases the clock speed down to 600MHz---
half of the maximum 1.2GHz---so that the CPU's temperature stays at a
safe level.
We found that without proper cooling solutions (heatsink or fan), 
prolonged use of the system would result in CPU frequency decrease
that may affect evaluation.

Another factor to consider is power supply. From our experiences, the
Pi 3 frequency throttling also kicks in when the power source can not
provide the required minimum of 2A current.
In experiments conducted with a power supply that only provided 1 Amp,
the Pi was unable to sustain a 1.2 GHz clock speed, and instead,
fluctuated between operating at 600 MHz and 1.2 GHz. As a result, it
is necessary, or at least highly recommended, that the power supply
used for the Raspberry Pi 3 be capable of outputting 2 Amps, otherwise
optimal performance isn't guaranteed.

Our initial experiment results suffered from these issues, after which
we always carefully monitored the current operating frequencies of the
CPU cores during the experiments to ensure the correctness and
repeatability of the results.

